Mathematical Analysis of Path MTU Discovery With New Generation Networks

In this paper we have presented the effects of path mtu discovery in IPv4 & IPv6 in mathematical, logical and graphical representation. We try to give a mathematical model to the working of path mtu discovery and calculated its behaviour using a transmission of a packet. We analysed the time consumed to transmit a single packet from source to destination in IPv6 network in the presence of PMTUD and similarly in IPv4 network with DF bit 1. Based on our analysis, we concluded that the communication time increases with the varying MTU of the intermediate nodes. Moreover, we formulated the mathematical model to determine the communication delay in a network. Our model shows that the asymptotic lower bound for time taken is $\Omega(n)$ and the asymptotic upper bound is $\Theta(n^2)$, using PMTUD. We have find that the packet drop frequency follows the Bernoulli's trials and which helps to define the success probability of the packet drop frequency, which shows that the probability is higher for packet drop rate for beginning $2\%$ of the total nodes in the path. We further found that $^{n}C_{a}$ possible number of a-combinations without repetitions that can be formed for a particular number of packet drop frequency. The relation between summation (acts as a coefficient in the time wastage equation) of each combination and their frequency resulted in symmetric graph and also mathematical and statistical structures to measure time wastage and its behaviour. This also helps in measuring the possible relative maximum, minimum and average time wastage. We also measured the probability of relative maximum, min and average summation for a given value of packet drop frequency and number of nodes in a path.

==> liter-intro.tex <==
\section{Literature Overview}
\label{sec:overview}
Thiago Lucas et al. \cite{flowfragment} carried out an analytic study of comparing the IPv4 \& IPv6 network using Path MTU Discovery in UDP protocol. The study concentrates on the effect of the Path MTU Discovery in datagram transmission in both the networks, by allowing and disallowing the fragmentation under UDP protocol. In this study, the jitter and the bandwidth are taken as the parameters to analyse the effectiveness of the two protocols with respect to the size of the datagram. The size of transmitting datagram is varied from 100 KB to 5 MB. The results of the comparison illustrated a great variation in IPv4 network and a minor changes in IPv6 network w.r.t. the two parameters. In IPv4, the jitter doubled and the bandwidth halved in case of no fragmentation as compared to the fragmentation. While in IPv6 network, the jitter and the bandwidth shows minor changes. Additionally, there is a reverse effect as compared to IPv4 network i.e., the jitter decreased and the bandwidth increased on the datagrams with restricted fragmentation as compared to unrestricted fragmentation of datagrams. This study focused on the effect of PMTUD on both the protocols using virtual network environmental simulations.

Matthew Luckie \& Ben Stasiewicz in \cite{behave} measures the Path MTU Discovery behaviour for 50 thousand popular websites by measuring the TCP behaviour after the PTB messages reached the host asking to send smaller packets. The authors concluded that the failure of the PMTUD infers to no response from the host to reduce the packet size or to clear the DF bit for tree consecutive times upon sending the PTB messages by remote TCP connection \cite{behave}. They depicted that the failure rate, as predicted in the previous studies for the IPv4, is much lesser than what is stated. It shows that nearly 80\% of the devices act normally on PTB messages for both IPv4 \& IPv6 \cite{behave}. They identified that most of the failure rate is due to the software bugs rather than filtering by the firewalls. Nearly, 62\% of the PMTUD failure rate can be reduced if focused on correcting these software bugs. This study found out that 11\% of web-servers limit themselves to packets with size no longer then 1380 bytes. On basis of this analysis, they proposed three different strategies to cutoff the failure rate in IPv4. First, the operating systems that refuses to lower the packet size below the threshold limit, should set the DF bit, if the path MTU is lower than the threshold limit \cite{behave}. Second, to debug the middleboxs that alter the TCP MSS size to 1380 bytes to ensure the correct forwarding of the PTB messages by identifying their manufactures \cite{behave}. Third, to make aware the system administrator of the importance of forwarding the PTB messages. While this study doesn't present any mathematical modelling or insight chemistry of the Path MTU Discovery on IPv6 network, rather it focuses on the causes for failure of PMTUD in IPv4 \& IPv6 based on TCP behaviour after PTB message are send to host \cite{behave}.

Christopher A. Kent \& Jeffrey C. Mogul \cite{frag} presented the study that changed the whole perspective of the packet transmission, giving rise to the usage and dependency on Path MTU Discovery by suggesting to set the DF bit to $'1'$. In this study, they found out the misuse of fragmentation by hackers and also a factor responsible for the poor performance and quality of the service. Another retrospection on the similar behaviour \cite{retro}, is published by the same authors stating the  further need of improvement of the PMTUD type techniques for reducing the harm that the fragmentation is anticipating today. Both these studies discusses the harm due to fragmentation and promoting the techniques like PMTUD to lower the harms that the fragmentation can cause. Similar work by F. Gont et al. \cite{rfc8021} suggesting to take out the IPv6 atomic fragmentation on the upcoming revision of the core IPv6 protocol specification by stating that \enquote{Its of no real gain and this kind of functionality is undesirable}. They further stated that, this can result in several security vulnerabilities in IPv6 by misusing the atomic fragmentation and  causes interoperability issues with other protocols relying on it. Nearly 57\% of the web-servers that are tested, fail to generate the IPv6 atomic fragments as per the ICMPv6 messages with a size of MTU lower then the 1280 bytes resulting an interoperability issues between the different protocols in the IPv6 stack \cite{rfc8021}.

Matthew Luckie et al. in \cite{firewall} carried out an analysis of Path MTU Discovery in IPv4 network. In this analysis, they have tried to resolve the failure of the PMTUD in modern network system. This study discusses and presents some important issues related to the cause of the failure of PMTUD in IPv4 network. They have presented a detailed analysis on inferring the exact location of the each failure of PMTUD \cite{firewall}.

K. Lahey \cite{rfc2923} presented a draft in IETF that includes the study of several TCP implementation issues with PMTUD. In this study, they presented three problems, namely black hole detection, stretch ACK due to PMTUD, and determining MSS from PMTU. With the explanation of these issues they have given detailed analysis for resolving them. The main motivation of this study is to improve the current conditions of the internet by improving the efficiency and quality of TCP/IP implementation.

\section{Motivations}\label{sec:motive}
We have gone through all of the literature that came in our way through the Search Engine like google and from Libraries using keywords "MTU or Maximum Transmission Unit" , "Path MTU Discovery or PMTUD", "Mathematical modeling/behaviour/aspects/structures of/in Path MTU discovery", "performance/analysis/evaluation of/in PMTUD" and "Surveys/reviews/study on Path MTU Discovery" and also related keyword but we haven't found any resembled or close resemble of the work which we have presented in this paper and most of them are surveys and a review on the behaviour/performance/analysis of Path MTU Discovery in the internet systems, parameters and the components. It was shocking to know that no study in the past has presented the mathematical modeling of the Path MTU Discovery for sending a packet from a source to destination. This paper presents a novel study of showing how that Path MTU discovery exhibits mathematical structure to explain possible performance and behaviour of latency in PMTUD in IPv4 and Ipv6 network. How this study can be harnessed? And what we can gather from this is all depends on how readers can utilize it but we try to give a possible sketch of its applications below:
\begin{itemize}
    \item Pre-examination of the latency in a network running Path MTU Discovery using mathematical modeling.
    \item Measuring the robustness of similar proposed techniques in terms of latency with the Path MTU Discovery.
    \item Using the mathematical models in designing a better simulators that will mimic the real world performance.
    \item Used to compare and measure the network parameters of the proposed method with state-of-the-art Path MTU Discovery when the implementation of the method is not possible in the node. 
\end{itemize}

This work is based on theoretical experiments using proofs and case study which can be used in verifying the new methods, schemes, and algorithms for testing the robustness of the newly proposed methods/schemes/techniques with the start-of-the-art PMTUD algorithm. This would be best fit when the schemes or methods is impossible for the authors to implement it in the node/router due to vendor's side restrictions and because of no open source platform to test the method/algorithm/scheme with the path mtu discovery to get the experimental results. Therefore this study can be used to compare the network parameters of the proposed methods with path mtu discovery using $Matlab$ or similar mathematical simulators by following the benchmarking methodologies given by Bradner et al. in \cite{bench1, bench2}, like we have used in \cite{HUSSAIN2021} for our new proposed algorithm called Dynamic MTU for reducing the packet drop and time delay associated in path MTU Discovery as defined in its preprint \cite{hussain2020measuring}. We strongly believe that this study can be harnessed to design a better protocols and techniques which can replace Path MTU Discovery by solving and tackling the root problems in the Path MTU Discovery protocol, which we tried to define in this paper.
